Towards Automatic Discovery of Cybercrime Supply Chains

Cybercrime forums enable modern criminal entrepreneurs to collaborate with other criminals into increasingly efficient and sophisticated criminal endeavors. Understanding the connections between different products and services can often illuminate effective interventions. However, generating this understanding of supply chains currently requires time-consuming manual effort. In this paper, we propose a language-agnostic method to automatically extract supply chains from cybercrime forum posts and replies. Our supply chain detection algorithm can identify 36% and 58% relevant chains within major English and Russian forums, respectively, showing improvements over the baselines of 13% and 36%, respectively. Our analysis of the automatically generated supply chains demonstrates underlying connections between products and services within these forums. For example, the extracted supply chain illuminated the connection between hack-for-hire services and the selling of rare and valuable `OG' accounts, which has only recently been reported. The understanding of connections between products and services exposes potentially effective intervention points.

==> Acknowledgement.tex <==
\section*{Acknowledgments}
% Names should be here.
Moore-Sloan?

==> Classification.tex <==
% \section{Classification}
% \label{classification}
% In this section we describe the two supervised classification tasks and the separate pipelines developed to solve them. This section will discuss the feature extraction, model selection and performance evaluation process of the separate classification tasks. 

% \subsection{Classifiers}

% We tested the following four classification algorithms for both the product and reply classification tasks: 1) FastText, 2) Logistic Regression, 3) SVM, 4) XGBoost. We tuned each of these methods to reduce over-fitting of our labeled data~\cite{Chen:2016:XST:2939672.2939785,DBLP:journals/corr/JoulinGBM16}. We selected these four classifiers as a diverse set of classifier types but we did not test an exhaustive set of classification methods. Further exploration could be done which might identify better performing classification algorithms for each task.

% \subsection{Feature Extraction}
% The text considered in both the product and reply classification tasks were the actual full post content. Primary post processing applied to the text was to remove stop words by using English and Russian stop word dictionaries. We extracted features using the TF-IDF algorithm ~\cite{Baeza-Yates:1999:MIR:553876} to produce a vector where each element corresponds to that terms' TF-IDF score a particular post. We experimented with n-grams built on characters, and words. Character n-grams outperformed word with both Hackforums and Antichat and so we used character n-grams when generating TF-IDF vectors. It is important to note that TF-IDF was used on all models but FastText which had a built-in feature extraction methodology. The additional processing applied before performing TF-IDF, was dependent on the classification task and is as follows. 

% \paragraph{Products:}
% The product classification task is to differentiate the first post in a thread into one of 14 categories listed in Table~\ref{table:product_annotation_labels}.
% We include the title of the thread along with the contents of the initial post in product classification because the thread title often contains additional information about the product advertised in the post body. For Antichat, we under-sampled the \texttt{account} category so that it would be 90\% the size of the \texttt{other} category. \dm{Ilia can you describe this text better?}

% \paragraph{Replies:}
% The reply classification task is to differentiate the replies into one of eight categories list in Table~\ref{table:reply_annotation_labels}.
% We applied a quoted text removal algorithm so that our classifiers would not mistake the actual reply content from someone quoting another post in the same thread. Our algorithm traversed each thread in order of time replied and kept track of all the seen replies. On every new reply, it removed the first instance of each previous reply. After the algorithm finished removing quotes from a thread, it cleared its cache of seen replies and starts over with a new thread. In order for a reply to be removed, the entire post text had to exactly match, case and punctuation included. Despite the (small) risk of a reply containing the entire text of a previous reply in the same thread by coincidence rather than quotation, we chose this algorithm for its forum agnosticity. Risk of text incorrectly removed text from a reply was determined small because 1) the median number of replies per thread was 3 for Antichat and 4 for Hackforums, both short enough to make duplicates unlikely, and 2) the main response typically affected is one following a single word reply: "vouch" with no punctuation.

% \subsection{Classification Evaluation}
% We performed stratified 5-fold validation of each classification algorithm since our classes were highly imbalanced. For highly imbalanced datasets, normal k-fold cross validation often produces a biased evaluation because the limited number of folds generated can have biased class distributions. Stratified k-fold validation is recommended in these instances since it ensures an ``apples-to-apples'' evaluation where the same distribution of the target values that existed in the main data set are maintained for each fold~\cite{SCV}.

% The difficulty of cross domain prediction was outlined in Durrett, et al.~\cite{Durrett2017IdentifyingPI}. Therefore, we generate a separate model for each forum that is unlikely to perform well on other forums. In order to build a well performing classifier for a new forums, it would likely require the labeling of around 4,000 -- 6,000 posts by a domain expert fluent in the language of the forum based on the learning curves in Figures~\ref{fig:product_learning_curves_english} and \ref{fig:product_learning_curves_russian}.  It is important to note that the resulting weighted F1 scores were based on classifying all the product categories listed in Table~\ref{table:product_annotation_labels} including \textit{other}. We chose to include the \textit{other} label in the learning curves because it would be categorized when classifying the remaining data.

% It is important to mention individual precision metrics to indicate which classes are the easiest to predict and which are the most difficult. In the Logistic Regression reply classifier, all three categories across datasets have precision scores over 0.80. The most precise reply category is \texttt{selling} across both datasets and we hypothesize this is due to the occational ambiguity of \texttt{bought} replies appearing like \texttt{other} replies. Furthermore in the XGBoost Product classifiers top three categories in Hackforums in terms of precision are \texttt{crypter}, \texttt{hacked-server}, and \texttt{traffic}. The top performers 


% \begin{table*}[!t]
% \centering
% \begin{tabular}{@{}lrr@{}}
% \toprule
%                      & \multicolumn{1}{c}{\textbf{Antichat}} & \multicolumn{1}{c}{\textbf{Hackforums}} \\ \midrule
% \textbf{Top Reply}   & selling (0.890)                       & selling (0.893)                         \\
% \textbf{Low Reply}   & bought (0.860)                        & bought (0.828)                          \\
% \textbf{Top Product} & crypter (0.905)                       & crypter (0.832)                         \\
% \textbf{Low Product} & other (0.502)                         & spam-tool (0.497)                       \\ \bottomrule
% \end{tabular}
% \end{table*}



% \begin{figure}[!htb]
%   \centering
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{images/classification/products_learning_curves_russian.png}
%     \caption{Product Classification Learning Curves Antichat (Russian)}
%     \label{fig:product_learning_curves_russian}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{images/classification/products_learning_curves_english.png}
%     \caption{Product Classification Learning Curves Hackforums (English)}
%     \label{fig:product_learning_curves_english}
%   \end{minipage}
% \end{figure}

% \begin{figure*}[!htb]
%   \centering
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{images/classification/XGBoost-russian-CM-text-char-other.png}
%     \caption{Russian Product Classification XGBoost Confusion Matrix}
%     \label{fig:russian_product_cm}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{images/classification/XGBoost-english-CM-full_text-char-other.png}
%     \caption{English Product Classification XGBoost Confusion Matrix}
%     \label{fig:english_product_cm}
%   \end{minipage}
% \end{figure*}

% The graphs in figures \ref{fig:russian_product_learning_curve} and \ref{fig:english_product_learning_curve} are weighted F1 scores where scores are calculated for each label and averaged by the number of true instances in each label. 

% When determining which model to use we actually introduced a weighted precision metric. This score was a weighted average of the precision scores across all the different categories, besides \textit{other}. We ignored the \textit{other} class because we are not concerned with having a high or low precision in that category or how that category's score affects the overall weighted precision. Although other classifiers perform equally as well as XGBoost in weighted F1 scoring, we chose XGBoost for all product classification tasks because it always performs better in a non-weighted F1 scoring. We see similar out performance when considering weighted precision in Table \ref{table:precision_f1_scores}. The remaining Antichat and Hackforums product posts were classified using the \textbf{XGBoost} models.

% The second classification task useful for identifying supply chains is to categorize the replies to the first post in a thread into eight categories. We chose the categories based on subject matter expertise to best separate posts which describe a spectrum of interest in the advertised product. We did not consider this a binary classification problem because of the uniqueness of the posts where someone is signaling interest. In other words, considering this a binary classification problem would over-generalize a complex marketplace environment. 

% The same dominant model result is not present in the reply classification task and we can see this from just figures \ref{fig:russian_reply_learning_curve} and \ref{fig:english_reply_learning_curve}. Antichat's highest performing reply classifier, in terms of weighted F1, is XGBoost with a score of 0.733 when trained on all the annotated data. In Hackforums, FastText had the highest weighted F1 of 0.705. Finding the best classifier is even less obvious when consulting Table \ref{table:precision_f1_scores} where the \textbf{SVM} in Antichat had the highest weighted precision and the \textbf{Logistic Regression} \is{Beware, a lot of questions will come and question the model selection. Can we somehow claim that the performance is the same as models capable of capturing more complex interactions?}\ma{Im not sure what this means. More complex interactions?} model had the highest weighted precision for Hackforums. Ultimately, we used the later two to classify the remaining replies by relying on the models with the highest weighted precision. This is because although we care about overall model performance, we want to ensure the integrity of our supply chain links, described later, and a higher precision would ensure that. In other words, we decided to trade recalling potential classification for the legitimacy of the classifications the models made. 


% \begin{table*}[!t]
% \centering
% \begin{tabular}{@{}lrllcllclllll@{}}
% \toprule
%                              & \multicolumn{6}{c}{\textbf{Antichat}}                                                                                                                 & \multicolumn{6}{c}{\textbf{Hackforums}}                                                                                                               \\ \midrule
%                              & \multicolumn{3}{c}{\textit{Product}}                                           & \multicolumn{3}{c}{\textit{Reply}}                                   & \multicolumn{3}{c}{\textit{Product}}                                 & \multicolumn{3}{c}{\textit{Reply}}                                             \\
% \textbf{Model}               & \multicolumn{1}{c}{Prec} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & Prec           & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & Prec           & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Prec} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} \\ \midrule
% \textbf{FastText}            & 0.824                    & 0.734                       & 0.764                  & 0.823          & 0.318                       & 0.450                  & 0.722          & 0.582                       & 0.627                  & 0.800                   & 0.427                        & 0.539                  \\
% \textbf{Logistic Regression} & 0.831                    & 0.718                       & 0.753                  & 0.874          & 0.245                       & 0.381                  & 0.617          & 0.564                       & 0.617                  & 0.852                    & 0.363                       & 0.492                  \\
% \textbf{SVM}                 & 0.817                    & 0.748                       & 0.767                  & 0.654          & 0.213                       & 0.301                  & 0.716          & 0.578                       & 0.614                  & 0.812                    & 0.332                       & 0.440                  \\
% \textbf{XGBoost}             & 0.824                    & 0.677                       & 0.729                  & 0.713          & 0.227                       & 0.328                  & 0.734          & 0.577                       & 0.627                  & 0.819                    & 0.352                       & 0.465                  \\ \bottomrule
% \end{tabular}
% \caption{Precision, recall and F1 scores of models across datasets and tasks with stratification}
% \label{table:precision_f1_scores_strat}
% \end{table*}

 


% \begin{figure}[!htb]
%   \centering
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{images/classification/replies_learning_curves_russian.png}
%     \caption{Reply Classification Learning Curves Russian}
%     \label{fig:reply_learning_curves_russian}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{images/classification/replies_learning_curves_english.png}
%     \caption{Reply Classification Learning Curves English}
%     \label{fig:reply_learning_curves_english}
%   \end{minipage}
% \end{figure}

% \begin{figure*}[!htb]
%   \centering
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{images/classification/reply-SVM-russian-CM-fulltext-char-other.png}
%     \caption{Russian Reply Classification SVM Confusion Matrix}
%     \label{fig:russian_reply_cm}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{images/classification/reply-Logistic-Regression-english-CM-fulltext-char-other.png}
%     \caption{English Reply Classification Logistic Regression Confusion Matrix}
%     \label{fig:english_reply_cm}
%   \end{minipage}
% \end{figure*}




% \subsection{Limitations}
% The annotated classes are extremely imbalanced and the annotated data is only based upon a subset of the entire ecosystem. \dm{By subset of the entire ecosystem do you mean we only analyzed two forums? If this is the case you should state this more clearly.} For this reason, although the annotations are based on subject matter expertise, they are biased toward certain classes and time frames. \dm{Is this because we only analyzed two forums over a fixed time period? If that is the case we should again state this more clearly. We should also say something about how our methods might extend to other forums. I.e., we would probably need to add new product categories and label more data due to the domain adaptation issues found in prior work.} We only tested a few common classifiers and reasonable features. Our classifiers could potentially be improved by identifying more useful features and exploring additional classifiers.
% %Another separate limitation we faced was from our inability to introduce deep learning based algorithms to perform this classification. This is because of the small amount of annotated data available for training\is{I am not sure how model selection relates to the dataset used? The story is -- we are already reporting results of less complex models?}. \ma{Not enough data to train a performant deep learning model} That being said, the simplicity and performance of non deep-learning based methods makes the models we chose for the classification tasks much more appealing for those interested in implementing. 
% Lastly, we did not obtain the same amount of annotations from both data sets. \dm{Why is this the case?}


==> Gang.tex <==
\section{Gang Detection}

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.49\textwidth]{Gang_clusters.png}
\caption{Graph with users as nodes and vouches as directed edges, with algorithm OpenOrd run on the graph.}
\label{fig:Gang_clusters}
\end{center}
\end{figure}

Figure \ref{fig:Gang_clusters} depicts a graph with users as nodes, and there is a directed edge between user A and user B if user A wrote a "vouch" reply on a thread initiated by user B. Users are categorized by the product that they most often sell, and edges are categorized by the category of the post in which that vouch was written. We ran the algorithm OpenOrd on this graph, and then hid the edges.

We can see many small clusters, and we can also see that many users are not in any cluster. The small clusters are gangs working together.

We define gangs as groups of about four to ten users working together to sell each others' products. As seen in the graph, some of the gangs contain users all in the same category, and some gangs contain users from a variety of categories.

We also ran the Modularity algorithm, and colored nodes by group detected by the algorithm. Many of the clusters detected by OpenOrd are in the same Modularity group. We consider these groups to be gangs.

Below we show the ForceAtlas 2 algorithm used to illustrate how the user reply network reflects our categories in Hackforums. What is ForceAtlas 2? Find out here: http://journals.plos.org/plosone/article?id=10.1371/journal.pone.0098679
\\
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.49\textwidth]{Hackforums_Graph_Users_as_Nodes.PNG}
\caption{Graph of Hackforums with Users as Nodes}
\label{fig:HF_Users}
\end{center}
\end{figure}
\\
\\
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.49\textwidth]{Hackforums_Graph_Users_as_Nodes_Zoom.PNG}
\caption{Zoomed in Graph of Hackforums with Users as Nodes}
\label{fig:HF_Users_Zoom}
\end{center}
\end{figure}
\\
Each node in Figure \ref{fig:HF_Users} represents a user. Figure \ref{fig:HF_Users_Zoom} is the same figure, zoomed in to exclude the nodes with few edges. Each edge represents a reply from one user to another within a post which belongs to a category indicated by the edge color:\\
\textcolor{video_game_service}{video game service, }
\textcolor{spam_tool}{spam tool, }
\textcolor{proxy}{proxy, }
\textcolor{botnet}{botnet, }
\textcolor{traffic}{traffic, }
\textcolor{DDoS_service}{DDoS service, }
\textcolor{crypter}{crypter, }
\textcolor{malware}{malware, }
\textcolor{hosting}{hosting, }
\textcolor{hacked_server}{hacked server, }
\textcolor{account}{account, } and
\textcolor{hack_for_hire}{hack-for-hire}. 

The color of each node represents the category that the corresponding user posted in most often, with the same color-coding.
\\
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.49\textwidth]{Hackforums_Graph_Posts_as_Nodes.PNG}
\caption{Graph of Hackforums with Posts as Nodes}
\label{fig:HF_Posts}
\end{center}
\end{figure}
\\
Each node in Figure \ref{fig:HF_Posts} represents a thread of at least 2 posts (each thread is an original post with any replies counted as additional posts in the same thread). An edge between two nodes represents a user in common, one who wrote a post in each thread. The nodes are colored by the category of the corresponding thread, with the same color-coding as Figure \ref{fig:HF_Users}. Each edge takes the color of its end-node in which its corresponding user posted earlier.

We then classified each reply to any post into one of three categories: potential/confirmed buyer, vouch, and other (clarifications, negative things), ignoring posts from the author of the original post. The classifier uses extreme-gradient-boosted trees and has an F1 score of about 75. We perform the following analysis on replies to posts manually classified into product categories.


==> Validation.tex <==
\section{Validation of classifiers and supply chains}
% Describing how the models hold up performance over time (or dont)
% Include an image of the confusion matrices (reply and product) that demonstrate the low precision in OTHER and high precision in the other labels
% Evaluation of supply chain links on annotated data
% https://www.overleaf.com/project/5bbe422fcad9855a2aac5277

% THIS PAGE SHOULDN'T EXIST
% SPLIT IT INTO THE METHODOLOGY SECTIONS
